Difference-based variance estimators with repeated measurements

In this paper, we formulate a general differencing framework for variance estimation across a range of settings. We demonstrate that conventional difference-based noise variance estimators cannot achieve the desired bias-correcting power in nonparametric regression with repeated measurements. A new high-order bias-corrected differencing scheme, adapted to repeated measurements, is proposed by interlacing inter-group and intra-group differencing. The theoretical properties of the new sequences and estimators are studied. Our proposals are particularly efficient in finite samples and under high signal-to-noise ratio scenarios, where asymptotic convergence has not yet fully taken effect, due to their strong bias-correcting power.

==> myPreliminary.tex <==
\usepackage{mathtools}
\usepackage{varioref} 
\ifnum\isXr=1\usepackage{xr-hyper}\fi
\RequirePackage[authoryear]{natbib} 
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\RequirePackage{graphicx}   
\usepackage{booktabs}
\RequirePackage{amsthm,amsmath}
\usepackage{natbib}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage{epsfig,amsmath,euscript,amsfonts}
\usepackage{array}
\usepackage{nccbbb}
\usepackage{verbatim}
\usepackage[lined,boxed,commentsnumbered, ruled,linesnumbered]{algorithm2e} 
\usepackage{graphicx}
\usepackage{bbm}
\usepackage{dsfont}
\usepackage{enumitem}
\usepackage{xfrac}
\usepackage{color}
\usepackage[utf8]{inputenc}
\usepackage{pdflscape}
\usepackage{tikz}
\usepackage{tikz-qtree}
\usetikzlibrary{arrows,shapes,trees,fit}
\usetikzlibrary{matrix}
\usepackage[cal=boondox]{mathalfa}
\usepackage{accents}
\usepackage{marginnote}
\usepackage{xcolor}
\usepackage{todonotes}

\usepackage{lipsum}
\usepackage{float}
\usepackage{relsize}
\usepackage{accents}
\usepackage{multirow}
\usepackage{lscape}
\usepackage{bbold}
\usepackage{comment}
\usepackage{caption}
\usepackage{xcolor}
\allowdisplaybreaks
\usepackage{makecell}
\setcellgapes{2pt}
\usepackage{cancel}
\usepackage{textcomp}
\usepackage{adjustbox}
\usepackage{algorithm2e, algorithmic}
\usepackage{pifont}

\theoremstyle{plain}
\newtheorem{axiom}{Axiom}
\newtheorem{claim}[axiom]{Claim}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{example}{Example}
\newtheorem*{fact}{Fact}
\newtheorem*{remark}{Remark}
\theoremstyle{remark}
\newtheorem{case}{Case}

\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\vech}{\mathop{\mathrm{vech}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\mean}{mean}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\logit}{logit}
\DeclareMathOperator{\expit}{expit}
\newcommand\norm[1]{\left\lVert#1\right\rVert}
\newcommand{\comp}{\textsc{comp}}
\newcommand{\T}{\textsc{T}}
\newcommand{\D}{\textnormal{d}}
\newcommand{\dd}{\,\textnormal{d}}

\newcommand{\pr}{\mathrm{pr}} 
\newcommand{\E}{E} 
\newcommand{\Cov}{\mathrm{cov}}
\newcommand{\Var}{\mathrm{var}}
\newcommand{\bias}{\mathrm{bias}}
\newcommand{\Bias}{\mathrm{Bias}}
\newcommand{\Corr}{\mathrm{corr}}
\newcommand{\median}{\mathop{\mathrm{median}}}
\newcommand{\AMSE}{ {\mathrm{AMSE}}}
\newcommand{\SMSE}{ {\mathrm{SMSE}}}
\newcommand{\MSE}{ {\mathrm{MSE}}}
\newcommand{\CSD}{ {\mathrm{CSD}}} 
\newcommand{\Li}{ {\mathrm{Li}}}

\newcommand{\inD}{   \overset{ \textnormal{d}   }{\rightarrow} }
\newcommand{\inWPone}{   \overset{ \textnormal{wp1}   }{\rightarrow} }
\newcommand{\inAS}{   \overset{ \textnormal{a.s.}   }{\rightarrow} }
\newcommand{\inP}{  \overset{ \textnormal{pr}    }{\rightarrow} }
\newcommand{\inLp}{ \overset{ \mathcal{L}^p }{\rightarrow} }
\newcommand{\indep}{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern4mu{#1#2}}}
\newcommand{\eqD}{   \overset{ \text{$\mathcal{D}$}   }{=} }
\newcommand{\iid}{\textsc{iid}} 
\newcommand{\simIID}{   \overset{ \iid   }{\sim} }
\newcommand{\simIND}{   \overset{ {\indep}   }{\sim} }
\newcommand{\simApprox}{   \dot{\sim} }

\newcommand{\RV}{\textsc{rv}}
\newcommand{\cdf}{\textsc{cdf}} 
\newcommand{\cgf}{\textsc{cgf}} 
\newcommand{\pdf}{\textsc{pdf}} 
\newcommand{\pmf}{\textsc{pmf}} 
\newcommand{\chf}{\textsc{chf}} 
\newcommand{\mgf}{\textsc{mgf}}
\newcommand{\EF}{\textsc{EF}}
\newcommand{\NEF}{\textsc{NEF}}
\newcommand{\MLE}{\textsc{MLE}}
\newcommand{\JS}{\textsc{JS}}
\newcommand{\MAP}{\textsc{MAP}}
\newcommand{\Med}{\textsc{Med}}
\newcommand{\MME}{\textsc{MME}}
\newcommand{\GMME}{\textsc{GMME}}
\newcommand{\minimax}{\textsc{M}}
\newcommand{\Bayes}{\textsc{Bayes}}
\newcommand{\Adm}{\textsc{A}}
\newcommand{\HPD}{\textsc{HPD}}
\newcommand{\ET}{\textsc{ET}}

\newcommand{\Bern}{\textnormal{Bern}} 
\newcommand{\Unif}{\textnormal{Unif}} 
\newcommand{\Logistic}{\textnormal{Logistic}} 
\newcommand{\Normal}{\textnormal{N}} 
\newcommand{\logNormal}{\textnormal{LN}} 
\newcommand{\Bin}{\textnormal{Bin}} 
\newcommand{\NB}{\textnormal{NB}} 
\newcommand{\HG}{\textnormal{HG}} 
\newcommand{\Geom}{\textnormal{Geom}} 
\newcommand{\Beta }{\textnormal{Beta}} 
\newcommand{\BetaBin}{\textnormal{Beta-Bin}}
\newcommand{\Ga}{\textnormal{Ga}} 
\newcommand{\Exp}{\textnormal{Exp}} 
\newcommand{\Expo}{\textnormal{Expo}} 
\newcommand{\Po}{\textnormal{Po}} 
\newcommand{\Multi}{\textnormal{Multi}} 
\newcommand{\Wishart}{\textnormal{Wishart}} 
\newcommand{\MIG}{\textnormal{MIG}} 
\newcommand{\student}{\textnormal{t}} 
\newcommand{\Cauchy}{\textnormal{Cauchy}} 
\newcommand{\Pareto}{\textnormal{Pareto}} 
\newcommand{\Laplace}{\textnormal{Laplace}} 
\newcommand{\Dir}{\textnormal{Dir}} 
\newcommand{\DP}{\textnormal{DP}} 
\newcommand{\Inv}{\textnormal{Inv-}} 
\newcommand{\F}{\textnormal{F}} 
\newcommand{\Supp}{\textnormal{Supp}} 
\newcommand{\round}{\textnormal{round}} 

\newcommand{\NBM}{\mathop{\mathrm{NBM}}}
\newcommand{\OBM}{\mathop{\mathrm{OBM}}}
\newcommand{\HOC}{\mathop{\mathrm{HOC}}}
\newcommand{\QS}{\mathop{\mathrm{QS}}}
\newcommand{\PSR}{ \textnormal{\tiny{P}} }
\newcommand{\TSR}{ \textnormal{\tiny{T}} }
\newcommand{\TRI}{ \triangle }

\def\estI{\textsc{i}}
\def\estII{\textsc{ii}}
\def\estIII{\textsc{iii}}
\def\DiffSeqMat{V}
\newcommand{\Long}{\textsc{r}}
\newcommand{\VB}{\textsc{r+}}
\newcommand{\DR}{\textsc{dr}} 
\def\Diag{\textnormal{Diag}}
\newcommand\tikzTextDist{1.1}
\newcommand\tikzTextMinDist{\tikzNodeDist/2}
\newcommand\tikzNodeDist{0.7}
\newcommand\tikzNodeMinDist{\tikzNodeDist/2}

\def\cusum{\textsc{cusum}}
\def\BAR{\textsc{bar}}
\def\TAR{\textsc{tar}}
\def\NAR{\textsc{nar}}
\def\AR{\textsc{ar}}
\def\ARMA{\textsc{arma}}
\def\MA{\textsc{ma}}
\def\BL{\textsc{bl}}
\def\GARCH{\textsc{garch}}
\def\ARCH{\textsc{arch}}
\newcommand{\ARE}{\mathop{\mathsf{ARE}}} 
\newcommand{\SOPR}{\textsc{sopr}} 
\newcommand{\BTC}{\textsc{btc}} 
\newcommand{\SPL}{\textsc{spl}} 
\newcommand{\KE}{\textsc{ke}} 
\newcommand{\TRACE}{\textsc{trace}} 


\usepackage{lineno}
\pagewiselinenumbers
\renewcommand\linenumberfont{\color{white}}

\makeatletter
\def\smallunderbrace#1{\mathop{\vtop{\m@th\ialign{##\crcr
   $\hfil\displaystyle{#1}\hfil$\crcr
   \noalign{\kern3\p@\nointerlineskip}
   \tiny\upbracefill\crcr\noalign{\kern3\p@}}}}\limits}
\makeatother

